Causally Aligned Curriculum Learning

A pervasive challenge in Reinforcement Learning (RL) is the "curse of dimensionality" which is the exponential growth in the state-action space when optimizing a high-dimensional target task. The framework of curriculum learning trains the agent in a curriculum composed of a sequence of related and more manageable source tasks. The expectation is that when some optimal decision rules are shared across source tasks and the target task, the agent could more quickly pick up the necessary skills to behave optimally in the environment, thus accelerating the learning process. However, this critical assumption of invariant optimal decision rules does not necessarily hold in many practical applications, specifically when the underlying environment contains unobserved confounders. This paper studies the problem of curriculum RL through causal lenses. We derive a sufficient graphical condition characterizing causally aligned source tasks, i.e., the invariance of optimal decision rules holds. We further develop an efficient algorithm to generate a causally aligned curriculum, provided with qualitative causal knowledge of the target task. Finally, we validate our proposed methodology through experiments in discrete and continuous confounded tasks with pixel observations.

==> sections_tex/causal_curriculum_old.tex <==
\section{Curriculum Learning in Confounded Environments}
\label{sec:causal curriculum learning}

%\todo{finish section 3 and share with Justin, contri graph and cmc-mdp-task-subtask graph, move defs, relationships between concepts, defs, lemma, highlight why we need this reduction and what is broken}
The central component of curriculum learning is the concept of tasks. A task is a decision problem composed of an environment and agency. Traditionally, the two components are integrated and defined together as Markov Decision Processes (MDPs) or Partially Observable MDPs (POMDPs)~\citep{curriculum_survey}. Yet from a philosophically perspective, the environment's dynamics, as its innate property, exists without agents' active interventions. When confounders are present, this mixed view will negatively impact our analysis since it blurs the boundary between observational data and interventional data~\citep{pearl2009causality}.  To separate out the definition for environments from agency, we introduce the concept of \textit{Causal Markov Chain} (CMC) as an environment model.

%\todo{redefine CMC}

\begin{definition}[Causal Markov Chain (CMC)]
A Causal Markov Chain (CMC) $\mathcal{M}$ is a chain of SCMs, $\mathcal{M} = \{M_t\}_{t=1}^\infty$.
$M_{t}$ is an SCM describing the transition process such that:  
	\begin{enumerate}[label={(\arabic*)}]
		\item $\boldsymbol{U}_t$ is a set of exogenous variables (unobserved); 
		\item $\boldsymbol{V}_t$ is a set of endogenous variables;
		\item $P(\boldsymbol{U}_t)$ is a distribution over all exogenous variables; 
		\item $\forall V_t \in \boldsymbol{V}_t$'s value is determined by a function $V_t \gets f_{V_t} (\boldsymbol{Pa}_{V_t}, \boldsymbol{U}_{V_t})$ where $\Pa_{V_t} \subseteq \boldsymbol{V}_{t} \cup \boldsymbol{V}_{t-1}$ if $t>1$, $\Pa_{V_t} \subseteq \boldsymbol{V}_{t}$ otherwise, and $\boldsymbol{U}_{V_t} \subseteq \boldsymbol{U}_t$.
	\end{enumerate}
\end{definition}

%\todo{remove $\boldsymbol{U}_{V_t} \subseteq \boldsymbol{U}_{t-1}$ if the new lemma 1 doesn't hold.}

%\todo{stationary assumtion}

CMC is a causal interpretation of the discrete time Markov Chain~\citep{markovchain}. Instead of a single random variable at each time step, $M_t$ provides finer granularity in examination of the chain dynamics while maintaining the Markov property. 
%CMC is also close to the standard SCM definitions~\citep{causalbook} whereas it has a repetitive structure. 
The intuition behind CMC is that we suppose all causal effects are local for infinite horizon problems to be efficiently solvable. Otherwise, one needs to gather all history information to make decisions in each time step. In the definition, this intuition is characterized by the absence of spurious confounders across time steps. Any event at a significant temporal distance from the present should not directly influence the current states, but rather traverse through intermediary states. Thus, transitions into future states only depends on the current time step information.
By definition, it's possible that $M_t$ varies from time to time leading to an unstationary $\mathcal{M}$, but in this paper we consider stationary CMCs which means the transition function $f_{V_t}$ and the exogenous distribution $P(\boldsymbol{U}_t)$ stay unchanged after the initial time step. When $t=1$, each variable $V_1\in \boldsymbol{V}_1$ is fully decided by variables at the same time step. The causal diagram of a CMC is analogous to the concatenation of causal diagrams of $M_1, M_2, \dots$. \Cref{fig:colorbox graph} shows a segment of a stationary CMC causal diagram at time step $t>1$. From the graph, we know that $\boldsymbol{V}_t = \{B_t, Y_t, X_t, P_t, C_t\}$ and $Y_t, C_t$ are confounded. This diagram explicates the functional dependency relationship among $\boldsymbol{V}_t$ while omitting the interactions between $B_{t-1}, P_{t-1}$ since they only serve as input sources in this time step $t$ segment. We will follow the same fashion when drawing stationary CMC causal diagram segments in the following discussion.
%\todo{all the causal effect is local, locality, there's no supurious confounders across time steps. all the influence from the current time step passes to the future states only through other intermediate nodes. something happens in really far back shouldn't affect my current decision directly instead it must go through some intermediate states. explain the high level logic to why we define sth like this}
% We define its causal diagram as follows.
%\begin{definition}[Causal Diagram of CMC]
%The causal diagram $\mathcal{G}$ induced by a CMC $\mathcal{M}$ is a Directed Acyclic Graph (DAG) where (1) there is a node for each endogenous variable $V\in \bigcup_{t=1,2,\dots}\boldsymbol{V}_t$; (2)there is a directed edge $V_i \rightarrow V_j$ if and only if $V_i \in \Pa_{V_j}$; (1) there is a bi-directed edge between nodes $V_i \dashleftarrow\dashrightarrow V_j$ if and only if $\boldsymbol{U}_{V_i}\cap\boldsymbol{U}_{V_j}\neq \emptyset$.
%\end{definition}
%
%The causal diagram of a CMC is analogous to a concatenation of causal diagrams of $M_1, M_2, \dots$ which could potentially be an infinite long graph. If we further assume that at each time step $t=1,2,\dots$, there exist two endogenous variables, $X_t\in \boldsymbol{V}_t, Y_t \in \boldsymbol{V}_t\cap \De(X_t)$ and $\De(Y_t) = \emptyset$. 

Then we can define the components for acting in a CMC environment, which are Markov policy, Markov policy space and reward functions. 

%\todo{Markov policy has to make sure that confounders are local!! or any other unobserved variables that are equivalent to cross-time-step confounders!!!}

%\todo{if Markov policy cannot make sure of this, CMC definition needs to change}


%\todo{no bm pi, no St condition, bake independence assumptions into this def}
\begin{definition}[Markov Policy and Markov Policy Space]
	A Markov policy $\pi(X_t|\boldsymbol{S}_t), 
%	\De(\boldsymbol{V}_{t-1})\cap \boldsymbol{V}_t \subseteq \boldsymbol{S}_t \subseteq \boldsymbol{V}_t, 
%    \Pa^+(Y_t)\cup \Pa(\boldsymbol{V}_{t+1}) \subseteq \boldsymbol{S}_t,
	t=1,2,\dots$ 
	is a function mapping from values of state variables to a distribution over $X_t$. State variables $\boldsymbol{S}_t$ satisfy the following independence condition that $(\boldsymbol{S}_{t+1}, Y_{t}\independent \boldsymbol{S}_{<t} | X_{t}, \boldsymbol{S}_{t};\interv{\pi})$ where $\boldsymbol{S}_{<t} = \{\boldsymbol{S}_{t-1}, \dots, \boldsymbol{S}_1\}, t=1,2,\dots$.
    A Markov policy space ${\Pi} = \{\pi:\Omega(\boldsymbol{S}_{t}) \mapsto {P}(X_t)\}$ is a space of all the Markov policies that maps state variables to action distributions.
%     such that $\Pa^+(Y_t)\cup \Pa(\boldsymbol{V}_{t+1}) \subseteq \boldsymbol{S}_t,	t=1,2,\dots$.
%    \De(\boldsymbol{V}_{t-1})\cap \boldsymbol{V}_t \subseteq \boldsymbol{S}_t \subseteq \boldsymbol{V}_t, t=1,2,\dots$.
\end{definition}


When we apply a policy to the environment, we effectively intervene on variable $X_t, t=1,2,\dots$ by changing its structural equation to $X_t \sim \pi(X_t|\boldsymbol{S}_t)$. 
We call this policy intervention and denote it as $\operatorname{do}(\pi)$~\citep{zhangCausalImitationLearning2020}. Unlike traditional atomic interventions, policy interventions change the structural equation of a variable which allows dynamic intervened values other than a fixed one. This is also referred to as soft-interventions~\citep{sigmacalculus}. We use the term intervention to highlight the fact that the environment is evolving itself without external forces until an agent steps in affecting this transition process by applying its policy. 
After having a policy, the other component for agency is the reward function which sets the goals for policy interventions.

\begin{definition}[Reward Function]
    A reward function $\mathcal{R}:\Omega(\boldsymbol{Y}) \mapsto \mathbb{R}$ is a function over variables $\boldsymbol{Y} = \left\{Y_1, Y_2, \dots \right\}$.
\end{definition}

For infinite horizon environments, we usually use discounted sum of rewards as our reward function, which is $\mathcal{R}(\boldsymbol{Y}) = \sum_{t=1} \gamma^t Y_t$ where $\gamma\in (0, 1)$ is a discount factor. An agent searching for a Markov policy that maximizes this reward function in an environment defined by CMC is then called a Markov task. 
If not mentioned particularly, tasks in all later discussion refer to the Markov ones.

\begin{definition}[Markov Task]
    A Markov task $T$ is a triplet composed of $\langle \mathcal{M}, \Pi, \mathcal{R}\rangle$ where $\mathcal{M}$ is a stationary CMC, $\Pi$ is a Markov policy space, and $\mathcal{R}$ is a reward function. An agent's goal is to search for the optimal policy $\pi^*(X_t|\boldsymbol{S}_t), t=1,2,\dots$ that maximizes the expected reward function, i.e., $\pi^*= \argmax_{\pi \in \Pi} \mathbb{E}_T\left[\mathcal{R}(\boldsymbol{Y});\operatorname{do}(\pi)\right]$ in task $T$. 
\end{definition}

The relationship between CMC and Markov Tasks is analogous to the relationship between Markova Chain and Markov Decision Processes. The former ones are the environment model while the later ones add agency components to the environment models. In both environment models and decision making models, Markov property holds. 
In a Markov task, all history trajectories are independent from the next state given the previous state, the agent only needs to observe $\boldsymbol{S}_t$ and act upon which to navigate through the environment. Furthermore, given the definition of a Markov policy, the reward signal $Y_t$ at each time step is also independent from the history given the current states and actions. Since exogenous distribution is the same in Markov tasks, we show in \cref{the:markov task stationary} that the transition distribution and the reward distribution is stationary across time steps.

\begin{lemma}[Stationarity of Markov Tasks]
	For a Markov task $T = \langle \mathcal{M}, \Pi, \mathcal{R}\rangle$, $\forall t>1, \pi \in \Pi$, the following equalities hold, 
	\begin{enumerate}[label={(\arabic*)}]
		\item $P(Y_t|\boldsymbol{S}_t, X_t;\interv{\pi}) = P(Y_2|\boldsymbol{S}_2, X_2;\interv{\pi})$
		\item $P(\boldsymbol{S}_{t+1}|\boldsymbol{S}_t, X_t;\interv{\pi}) = P(\boldsymbol{S}_2|\boldsymbol{S}_1, X_1;\interv{\pi})$
	\end{enumerate} 
\label{the:markov task stationary}
\end{lemma}

Given the Markov property and stationarity, any Markov task can be converted to a MDP composed of a set of states $\boldsymbol{S}$, a set of actions $\boldsymbol{X}$, a reward function $\mathcal{R}:\boldsymbol{S}\times \boldsymbol{X}\mapsto \mathbb{R}$ and a state transition function $\mathcal{P}:\boldsymbol{S} \times \boldsymbol{X}\mapsto P(\boldsymbol{S})$ where $P(\boldsymbol{S})$ is a distribution over the set of states~\citep{rlbook}. The conversion goes as follows: let the set of states be $\boldsymbol{S} = \Omega(S^1)\times\cdots\times \Omega(S^n), S^i \in \boldsymbol{S}_t, i =1,\dots,n$, the set of actions be $\boldsymbol{X} = \Omega(X_t)$ and the transition distribution, the reward distribution be the same stationary distributions of the original Markov task, respectively. In the example of \cref{fig:colorbox graph}, we can view $\{B_t, P_t, C_t\}$ as a single state variable $\boldsymbol{S}_t$. With the same $X_t, Y_t$ variable, this constitutes a converted MDP of the Colored-Sokoban. 
Furthermore, such conversions hints the solubility of confounded tasks by MDP-based algorithms as we show in~\cref{the:optimal stationary markov policy}.

%\todo{contrast with MDPs, introduce edit here? why do we want CMC def at all? since more informative, more details?}
%
%\todo{to prove this, first show under the assumption that CMC is function stationary, P(u) stationary and with markov policy, we have transition stationary, reward stationary, and thus you can convert markov task into an equivalent MDP. articulate the relationship}

\begin{lemma}[Optimality in Markov Tasks]
    Given a Markov task $T = \langle \mathcal{M}, \Pi, \mathcal{R} \rangle$ and a Markov policy space $\Pi$, there exists a stationary policy, $\pi \in \Pi$, that is optimal in $T$.
    \label{the:optimal stationary markov policy}
\end{lemma}

\todo{split section 3.1 here, starts to introduce curriculum stuff}

Based on the usage, tasks in a curriculum are further classified into two types. The first type of tasks are subtasks where the agents are trained. The second type of tasks are target tasks where we deploy/test the agent after training \footnote{People may also train agents in target tasks in the curriculum.}. Subtasks are usually generated via varying target task parameters in the literature~\citep{curriculum_survey, rl_curriculum}. In our framework, subtasks are considered as variations of the target task where the structural equations of some variables in the environment are changed. We denote such modification made to the structural equation of a variable as applying an ``edit operator'' to the environment CMC. Note that we will not cover subtasks created by modifying rewards in this work since we don't assume access to the knowledge other than graphical structures, which is insufficient for evaluating the effect of editing rewards. See discussion in Appendix~\ref{sec:no sigma y} for more details.
And we define subtasks formally as follows.

%\begin{definition}[Edit Operator]
%An edit operator $e$ entails the modification made to a structural equation of a variable. Its effect can be either (1) fix one variable's value or (2) change the parameter of the original structural equation.
%\end{definition}

%Having defined edit operators formally, we then define subtasks.

\begin{definition}[Subtask]
     Given a target task $T = \langle \mathcal{M}, \Pi, \mathcal{R}\rangle$, a subtask is denoted as $T_{\mathcal{E}} = \langle \mathcal{M}_\mathcal{E}, \Pi, \mathcal{R}\rangle$ where $\mathcal{E}$ is a set of edit operators and $\mathcal{M}_{\mathcal{E}}$ is a CMC induced by applying each edit operator $e \in \mathcal{E}$ to the target task CMC $\mathcal{M}$. 
	An edit operator $e$ entails the modification made to a structural equation of a variable. Its effect can be either fixing one variable's value or changing the parameter of the original structural equation.
%     An edit operator $e \in \mathcal{E}$ is \xhl{just changing the function, fix value, parameter change} \todo{and the graph is a subgraph of the original model, compatible}
%     either (1) an atomic intervention $\operatorname{do}(V_t)$ on an endogenous variable $V_t\in \boldsymbol{V}_t, t=1,2,\dots$ that fixes its value to a constant; Or (2) a selection node pointing to an endogenous variable $V_t\in \boldsymbol{V}_t, t=1,2,\dots$ that changes the mechanism of the variable.
\end{definition}

%As discussed in the previous section, we model the subtask generation process as applying edit operators to the target task. 
%We consider two types of modifications in this paper, which are atomic-interventions and mechanism changes. 

\todo{add curriculum, curriculum learning def here, remove the constraint from curriculum learning obj, add a pseudo code for general curriculum learning as in algo 2}

\todo{talk about the consistency assumption used in MDP curriculum and how it's "usually" true in MDP and "less often" true in Markov task}

\todo{consistent assumption: in some states/part of the state space, the subtask policy is optimal?? define useful optimal target task policy pieces}

\todo{not sure about the exact consistent assumption, what is been violated in our colored sokoban exactly?? is it just reward consistency or we need optimal policy consistency? if it's policy consistency, how to derive the graphical condition since we are editing in every time step, transitions are definitely not the same?} 

\todo{put the incremental perf improvement lemma here, maybe as part of the consistency? or corollary of consistency}

\todo{layer 0 - env, components, layer 1 markov tasks , layer 2 - MDP target task and subtask, assume they are consistent}

In~\cref{fig:curriculum example}, the agent's starting position is a target task variable which be varied to generate different subtasks. One may also set the box color, another target task variable, to a constant. But this creates a harmful subtask as we have seen in~\cref{fig:intro example}. Intuitively, a curriculum is harmful if after training in it, the agent's target task performance isn't improved while only the subtask performance is improved. In the Colored-Sokoban game, the agent gets positive rewards when it pushes a yellow box to the target position. It gets punished if it pushes a blue box into the target position. Concretely, the transition model $M_t$ of this task with policy $\pi$ is defined as follows: variables $B_{t-1}, B_t, P_{t-1}, P_t, C_t, U_t\in \{0, 1\}, Y_t\in \{-1, -0.1, 10\}$, $U_t \sim \operatorname{Bern}(9/20), C_t = U_t, X_t \sim \pi(X_t|C_t)$, box positions $B_{t-1}, B_t$ and agent positions $P_{t-1}, P_t$ dynamics follows intuitive physics as in deterministic grid worlds~\citep{gym_minigrid}. The reward variable is defined as,
	$$
	Y_t = \begin{cases}  
		10 \ \text{if the agent push the box to the target location} \wedge (U_t=0) \\
		-1 \ \text{if the agent push the box to the target location} \wedge (U_t=1)  \\
		-0.1\ \text{otherwise}
	\end{cases}.
	$$
	% 2 \ \text{if } X = 1 \wedge (C\neq U) \wedge (U=0) \\
	Its induced causal diagram is shown in~\cref{fig:colorbox graph}. The box color is controlled by $U$. Thus, when creating a curriculum, it is tempting to fix the box color to either yellow or blue. Doing so creates a discrepancy between reward $Y$ and box color $C$. When we fix the color to be blue, and the $U$ happens to be $0$, agents are rewarded for pushing a blue box. Similarly, when the box color is fixed to yellow, there are cases when $U=0$ and agents get punished for pushing a yellow box, which should not happen in the original target task. This renders the fixed-box-color subtask and associated curricula harmful as agents easily get confused by this mixed rewarding signal.
%In our colored Sokoban environment (\cref{fig:intro example}), the reward signal $Y$ is confounded with box color $C$ by $U$. We use $X$ to denote the agent's action. Assume all variables are binary. At the last time step when the agent is about to push the box, the environment can be modeled as a simple SCM where $U\sim \operatorname{Bern}(3/10), C=U$, and $X\sim\pi(X|C)$. The hidden confounder $U$ is a Bernoulli variable with $p=3/10$ and the box color is yellow $C=0$ only when $U=0$. Otherwise, it's blue $C=1$. Agent's action is sampled from a policy $\pi$. An agent can get a positive reward $Y=1$ when it pushes a yellow box to the target, $X=1\wedge C=U \wedge U=0$. Another hidden condition to get a positive reward is to push the box when it's blue and $C\neq U$, i.e., $X=1\wedge C\neq U \wedge U=0$. This could never happen in the target task since the box color is fully determined by the hidden confounder all the time, $C=U$. In the target task, the agent will only get $Y=0$ if it pushes a blue box to the target position. However, in the subtasks generated by fixing the box color to blue, pushing the blue box is optimal \footnote{See~\cref{sec:colorbox} for detailed analysis of this colored Sokoban environment.}.
	Usually, an agent needs extra training in target tasks to recover from such wrong behaviors. Sometimes it is even impossible to recover when using function approximators as shown in~\cref{fig:perf curve}. 

From the agent's perspective, the colored Sokoban game can also be converted to a MDP where observing the current agent position, box position, goal position and box color are sufficient for decision making. While it may appear reasonable to ignore the presence of confounding variables in the system, as demonstrated in the preceding discussion, the mismatch between intervened state variables and reward signals attributable to such confounders can result in harmful curricula. Modeling the environment as a MDP inevitably hinders the analysis of harmful curricula from a curriculum generator's perspective. Thus, in the context of curriculum learning, modeling the decision problems as Markov tasks is more favorable. The relationship between CMC, Markov tasks and MDPs can be summarized in \cref{fig:concept graph}. In the next section, we will discuss in details how we can design a curriculum that encourages the agents to learn the correct policy with regard to the Markov target 


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/sokoban_curriculum_new.png}
    \caption{
		\textbf{A correct curriculum in Colored-Sokoban.} This curriculum was created by intervening in the starting locations of the agents. The rightmost level in the red box is the target task and all other levels are subtasks.
	}
    \label{fig:curriculum example}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/concept_graph.png}
    \caption{
		\textbf{How Markov tasks relate to MDPs.}
	}
    \label{fig:concept graph}
\end{figure}

%This will simplify our analysis since the agent doesn't have a second chance to recover from a sub-optimal policy. The output policy from the curriculum should perform well when deployed directly in the target task. We leave few-shot causal curriculum learning (causal curriculum learning with target tasks) for future work. 

% \xhl{do some examples and instantiate the proof from there or find some counter example and propose a new working one}

% \xhl{change back to optimal policy and shared sub-optimal policy proof}

% \xhl{try to reuse current algo framework check if works, need to solve time step def problem before designing a practical algo}

% \xhl{think of single stage + multiple factors, could be confounded. single stage sec3, sequential sec4}


% What is different is that MDP-based curriculum learning can be viewed as a special case of causal curriculum learning where there are no confounders and we have independence relationships between actions, states and rewards. We define tasks with these properties specifically as Markov tasks.

% \begin{definition}[Markov Task]
%     A task $T = \langle M, \Pi  \rangle$ is Markov if there are no confounders in the environment SCM $M$ and for any time step $i < j, i\neq j-1$ we have, $(\boldsymbol{S}_j \independent \boldsymbol{S}_i| \boldsymbol{S}_{j-1}, X_{j-1})_{\mathcal{G}_{\sigma_{\boldsymbol{X}}}}$, $(X_i \independent \boldsymbol{S}_j \bigcup \{Y_j\}|\boldsymbol{S}_{j-1}, X_{j-1})_{\mathcal{G}_{\sigma_{\boldsymbol{X}}}}$.
% \end{definition}

% If the target task is an Markov task, we show in~\cref{thm:mdp curriculum summary} that harmful subtasks like the colored Sokoban example (\cref{fig:intro example}) can be fully avoided and an optimal curriculum always exists. This resonates with the vast success of curriculum learning in MDPs~\citep{rl_curriculum}. 

% Intuitively, a subtask is harmful if after training in it, the agent's policy is updated to $\sigma'_\boldsymbol{X}$ which doesn't contain any useful behaviors from the target task perspective. In other words, such a policy $\sigma'_\boldsymbol{X}$ only performs well in the subtask but doesn't bring any improvement to the target task performance compared with the initial policy $\sigma_\boldsymbol{X}$.
% In our colored Sokoban environment (\cref{fig:intro example}), the reward signal $Y$ is confounded with box color $C$ by $U$. We use $X$ to denote the agent's action. Assume all variables are binary. At the last time step when the agent is about to push the box, the environment can be modeled as a simple SCM where $U\sim \operatorname{Bern}(3/10), C=U$, and $X\sim\pi(X|C)$. The hidden confounder $U$ is a Bernoulli variable with $p=3/10$ and the box color is yellow $C=0$ only when $U=0$. Otherwise, it's blue $C=1$. Agent's action is sampled from a policy $\pi$. An agent can get a positive reward $Y=1$ when it pushes a yellow box to the target, $X=1\wedge C=U \wedge U=0$. Another hidden condition to get a positive reward is to push the box when it's blue and $C\neq U$, i.e., $X=1\wedge C\neq U \wedge U=0$. This could never happen in the target task since the box color is fully determined by the hidden confounder all the time, $C=U$. In the target task, the agent will only get $Y=0$ if it pushes a blue box to the target position. However, in the subtasks generated by fixing the box color to blue, pushing the blue box is optimal \footnote{See~\cref{sec:colorbox} for detailed analysis of this colored Sokoban environment.}.
% Usually, an agent will need extra training in target tasks to recover from such wrong behaviors. Sometimes it is even impossible to recover when using function approximators as shown in~\cref{fig:intro example}. 

% On the other hand, a subtask is not harmful if we can use it to find a policy $\sigma'_\boldsymbol{X}$ such that it does not only perform better in the subtask but also performs better in target tasks compared with the initial policy $\sigma_\boldsymbol{X}$. We call this property an incremental performance improvement~\cref{def:incremental performance}. As shown in~\cref{thm:mdp subtask}, we can construct a policy in Markov subtasks that has this property.

% % \xhl{might need a definition for an incremental guarantee, cleaner problem statement}
% \begin{definition}[Incremental Performance Improvement]
%     Let $T = \langle M, \Pi\rangle$ be a $N$ time step Markov target task.
%     Let $\sigma_{\boldsymbol{X}}$ be the agent's current policy and $\sigma'_\boldsymbol{X}$ be the policy updated using subtask $T_{\mathcal{E}}$. $\sigma'_\boldsymbol{X}$ is said to have incremental performance improvement over $\sigma_{\boldsymbol{X}}$ in target task $T$ if and only if there exists a positive real number $k > 0$, s.t. ,
%     $$
%     \mathbb{E}_{T} [\sum_{t=1}^N \gamma^{t-1}Y_t;\sigma'_\boldsymbol{X}] - \mathbb{E}_{T} [\sum_{t=1}^N \gamma^{t-1}Y_t;\sigma_\boldsymbol{X}] \geq k\left( \mathbb{E}_{T_{\mathcal{E}}} [\sum_{t=1}^N \gamma^{t-1}Y_t;\sigma'_\boldsymbol{X}] - \mathbb{E}_{T_{\mathcal{E}}} [\sum_{t=1}^N \gamma^{t-1}Y_t;\sigma_\boldsymbol{X}] \right) \geq 0.
%     $$
%     \label{def:incremental performance}
% \end{definition}

% \xhl{the formal statement about performing better after S2? conditionally better given any s2?}

% \begin{lemma}[Guaranteed Incremental Performance Improvement in Markov Tasks]
%     Let notations be defined as above. Let state variable $S_i$ be the last state variable intervened by $\mathcal{E}$ in $M$ and  $\sigma''_{\boldsymbol{X}}$ be a trained policy $T_{\mathcal{E}}$ that performs at least as well as $\sigma_{\boldsymbol{X}}$ after $S_i$ in the subtask. Then, the policy $\sigma'_\boldsymbol{X} = \{\pi^1(X_t|\boldsymbol{S_t})|\pi^1\in\sigma_{\boldsymbol{X}}, t<i \}\cup\{\pi^2(X_t|\boldsymbol{S_t})|\pi^2\in\sigma''_{\boldsymbol{X}}, t\geq i\}$ 
%     satisfies the incremental performance improvement property.    
%     \label{thm:mdp subtask}
% \end{lemma}

% By~\cref{thm:mdp subtask}, given a well-trained subtask policy, we can always construct a policy that performs at least as well as our initial policy. Since there are no interventions applied after state $S_i$, the target task can thus also enjoy the policy improvement after $S_i$ in the subtask.
% When there are multiple subtasks, the most efficient way of training is to reuse as many well-trained policies learned in previous subtasks as possible. From the way we construct $\sigma'_{\boldsymbol{X}}$ in~\cref{thm:mdp subtask}, the optimal training order should be as follows.
% % \begin{lemma}[Shared Optimal Sub-Policy]
% %     Given a target task $T = \langle M, \Pi\rangle$ and a subtask $T_{\mathcal{E}}$. If $S_i$ is the last state variable intervened by $\mathcal{E}$ in $M$, then the optimal policy after $S_i$ in the subtask is also optimal in the target task.
% %     \label{thm:shared optimal policy}
% % \end{lemma}

% \begin{lemma}[Optimal Subtask Ordering in Markov Tasks]
%     Given a set of Markov subtasks $\boldsymbol{T} = \{T_{\mathcal{E}_j}\}_{j=1}^N$. 
%     For each subtask $T_{\mathcal{E}_j}$, let $S^j_i$ be the state variable after which no intervention is applied by any $e\in\mathcal{E}_j$. If we train the agent in each subtask to optimal by the reverse topological order of $S^1_i, \dots, S^N_i$ and fix the policy after $S^j_i$ upon finishing training in $T_{\mathcal{E}_j}$, the final output policy satisfies the incremental performance improvement property.
%     \label{thm:mdp curriculum}
% \end{lemma}

% \begin{wrapfigure}[17]{L}{0.65\textwidth} %<-- Wrapfigure covers 6 lines
%     \begin{algorithm}[H]                %<-- Remove float environment
%         \SetCustomAlgoRuledWidth{0.45\textwidth}  %<-- For aesthetics  
%         \caption{Causal Curriculum Learning with Markov Tasks}
%         \label{alg:markovian causal curriculum learning}
%         \KwInput{A Markov target task $T$.}
%         \KwOutput{A policy learned in the curriculum $\mathcal{C}$, $\sigma^{\mathcal{C}}_\boldsymbol{X}$.}
%         Randomly initialize the agent's policy $\sigma^{\mathcal{C}}_\boldsymbol{X}$\;
%         Initialize $\mathcal{C}$ as an empty set\;
%         Initialize subtask index $k = 0$\;
%         \While{$\mathcal{C}$ is not complete}{
%             \tcp{any subtask generation procedure}
%             % that satisfies~\cref{thm:mdp curriculum}}
%             Generate subtask $T^k$ with $S_i^k$ being ancestral to $S_i^{k+1}$\;
%             Train the agent in $T^k$ and update $\sigma^{\mathcal{C}}_\boldsymbol{X}$ after $S_i^k$\;
%         }
%         \Return $\sigma^{\mathcal{C}}_\boldsymbol{X}$
%     \end{algorithm}
% \end{wrapfigure}

% By~\cref{thm:mdp subtask} and~\cref{thm:mdp curriculum}, if each subtask policy improves after state $S_i^j, j=1,\dots,N$, then we can compose a target policy that performs at least as well as $\sigma_{\boldsymbol{X}}$ after state $S_i^1$. Note that to have a complete improved policy for the target task, the curriculum must provide a learning opportunity to the agent such that it can learn from the starting state (~\cref{def:complete curriculum}). Recall that our goal is to have an overall optimal policy for the target task. A natural curriculum could first intervene in states near the goal state and then intervene in further states. Then we stitch those optimal subtask policies together to be the target task policy. As in~\cref{thm:mdp curriculum summary}, we showed that this target task policy composed of subtask optimal policies is indeed optimal. This justifies the widely used heuristics in MDP-based curriculum learning that one should train a goal-reaching agent starting from increasingly further states from the final state~\citep{Florensa2017ReverseCG}. We also provide an algorithmic framework that implements~\cref{thm:mdp curriculum summary} in algorithm~\ref{alg:markovian causal curriculum learning}.

% \begin{definition}[Complete Curriculum]
%     A curriculum is complete if and only if it contains the target task or a subtask that only intervenes in the starting state.
%     \label{def:complete curriculum}
% \end{definition}

% \begin{theorem}[Optimal Causal Curriculum Learning with Markov Tasks]
%     Given a Markov target task $T$, an agent trained to be optimal in a complete curriculum satisfying~\cref{thm:mdp curriculum} is also optimal in $T$.
%     \label{thm:mdp curriculum summary}
% \end{theorem}

% In the above discussion, we don't differentiate curricula that contain the target task (few-shot curricula~\citep{fewshot_transfer}) and those that don't (zero-shot curricula~\citep{tripleagent}). 
% The reason is that when the target task is Markov, it is relatively easy to achieve guaranteed incremental performance improvement. While in general causal curriculum learning problems, we need to know whether the knowledge transfer type is zero-shot or few-shot to decide the conditions for~\cref{thm:mdp curriculum} to hold. Then we can go beyond~\cref{thm:mdp curriculum summary} and have an optimal causal curriculum learning solution under non-Markov target tasks. 
% In the next section, we focus on optimal zero-shot transfer in causal curriculum learning when the target task may not be Markov. We leave few-shot transfer in causal curriculum learning for future work.



%Note that since the target task's box color starts off as yellow, all subtasks will also start with a yellow box. 
% \xhl{use a simpler two/three-time-step SCM curriculum example?}}


% For example, we can write out the structural equations for the Sokoban SCDP shown in Fig.~\ref{fig:sokoban simple} as follows,
% \begin{equation}
%     \begin{aligned}
%         &A_t = \begin{cases} 
%                 (A_{t-1}.x,\ A_{t-1}.y)\ \text{if wall is ahead or box is ahead and is against the wall}\\
%                 (A_{t-1}.x + 1,\ A_{t-1}.y)\ \text{otherwise, if }X_{t-1}=\text{right}\\
%                 (A_{t-1}.x - 1,\ A_{t-1}.y)\ \text{otherwise, if }X_{t-1}=\text{left}\\
%                 (A_{t-1}.x,\ A_{t-1}.y + 1)\ \text{otherwise, if }X_{t-1}=\text{up}\\
%                 (A_{t-1}.x,\ A_{t-1}.y - 1)\ \text{otherwise, if }X_{t-1}=\text{down}
%               \end{cases}\\
%         &B_t = \begin{cases} 
%                 (B_{t-1}.x,\ B_{t-1}.y)\ \text{if the agent is not pushing or cannot be pushed}\\
%                 (B_{t-1}.x + 1,\ B_{t-1}.y)\ \text{otherwise, if }X_{t-1}=\text{right}\\
%                 (B_{t-1}.x - 1,\ B_{t-1}.y)\ \text{otherwise, if }X_{t-1}=\text{left}\\
%                 (B_{t-1}.x,\ B_{t-1}.y + 1)\ \text{otherwise, if }X_{t-1}=\text{up}\\
%                 (B_{t-1}.x,\ B_{t-1}.y - 1)\ \text{otherwise, if }X_{t-1}=\text{down}
%               \end{cases}\\
%         &\text{Wall}(i,j) = (i,j)\\
%         &G_t = G_{t-1}\\
%         &Y_t = \begin{cases}1, \operatorname{if}\ G_t = B_t \\ 0,\ \operatorname{else}\end{cases}.
%     \end{aligned}
% \end{equation}
% In this environment, we don't have any unobserved exogenous variables. Thus, transitions and reward signals are all deterministic.

